Discourse Centric Evaluation of Machine Translation with a Densely Annotated Parallel Corpus

Several recent papers claim human parity at sentence-level Machine Translation (MT), especially in high-resource languages. Thus, in response, the MT community has, in part, shifted its focus to document-level translation. Translating documents requires a deeper understanding of the structure and meaning of text, which is often captured by various kinds of discourse phenomena such as consistency, coherence, and cohesion. However, this renders conventional sentence-level MT evaluation benchmarks inadequate for evaluating the performance of context-aware MT systems. This paper presents a new dataset with rich discourse annotations, built upon the large-scale parallel corpus BWB introduced in Jiang et al. (2022). The new BWB annotation introduces four extra evaluation aspects, i.e., entity, terminology, coreference, and quotation, covering 15,095 entity mentions in both languages. Using these annotations, we systematically investigate the similarities and differences between the discourse structures of source and target languages, and the challenges they pose to MT. We discover that MT outputs differ fundamentally from human translations in terms of their latent discourse structures. This gives us a new perspective on the challenges and opportunities in document-level MT. We make our resource publicly available to spur future research in document-level MT and the generalization to other language translation tasks.

==> old_intro.tex <==
\section{Introduction}
% Annotated corpora are important
Linguistically annotated corpora have contributed significantly to the advancement of key natural language technologies such as named entity recognition \citep{tjong-kim-sang-de-meulder-2003-introduction}, coreference resolution \cite{lee-etal-2017-end}, and discourse parsing \cite{surdeanu-etal-2015-two}.
% Monolingual corpora are not enough:
The majority of evaluation has, however, only been conducted on monolingual corpora such as the BBN name entity and pronoun coreference corpus~\cite{weischedel2005bbn}, the Penn Discourse Treebank~\citep{miltsakaki2004penn, webber2019penn}, and the OntoNotes corpus~\cite{weischedel-2013-ontonotes}.
And yet, languages differ considerably in terms of the range of discourse phenomena they exhibit. 
In particular, different languages have different linguistic features that influence the application of cohesive devices and there are language-specific constraints governing the choice of referring expressions.
For instance, \Cref{fig:intro_example} demonstrates a prominent feature that distinguishes Chinese and English -- it is a common practice in Chinese to omit pronouns (referred to as pronoun-dropping phenomenon), and an anaphoric link can be inferred from context without explicit assertion, as opposed to English, which does not allow the pronouns to be omitted.
Consequently, machine translation (MT) are presented with a significant challenge when producing correct explicit information on the target language when the source language does not require it. 

% The pros of our datasets: literature, long
% 1. General domain is not enough: we need literature domain
Another current hurdle in MT is the translation of well-structured discourse, such as novels, blogs and scientific texts.
To be a tad more specific, despite that machine translation systems have achieved satisfactory performance at translating individual sentences on the news domain~\cite{hassan-etal-2018-achieving}, they remain unsatisfactory when it comes to translating literary texts.
The reasons are two folded.
First, the majority of available parallel corpora contain sentence-level translations.





% 2. long: poses challenges for sentence-level systems.
% NMT progress
Machine translation (MT) has made significant progress in the past few decades.
Neural machine translation (NMT) models, which are able to leverage abundant quantities of parallel training data, have been one of the main contributors to this progress~\citep[][\textit{inter alia}]{transformer,junczys-dowmunt-etal-2018-marian}.
%Although NMT systems have achieved satisfactory performance at translating individual sentences and, they still show unsatisfactory results when translating scientific and technical text.
Unfortunately, the majority of available parallel corpora contain sentence-level translations. %, where sentences are not continuous but rather independent.
As a result, models trained on these corpora translate text quite well at the sentence level, but perform poorly when the entire document translation is seen in context \citep{voita-etal-2019-good, werlen2021discourse}.
%\textcolor{red}{TODO: citation needed}
%in a sentence-by-sentence fashion.
% But Discourse matters:
    % document translation is more than sentence-by-sentence translation, i.e. discourse phenomena
    % which NMT systems have hard time dealing with. (example)
%However, document translation is more than sentence-by-sentence translation. 
Particularly, sentence level translation models %the advantage of improving efficiency, but with 
 tend to omit relevant contextual information, resulting in a lack of coherence %and cohesion 
in the produced translation. 
For example, in \Cref{fig:intro_example}, the sentence-level MT system fails to capture discourse dependencies across sentences and the same concepts are not consistently referred to with the same translations (i.e. \orangeEnt{Weibo} vs \orangeEnt{micro-blog}, \redEnt{Qiao Lian} vs \redEnt{Joe} vs \redEnt{Joe love}).\footnote{This discourse phenomenon is referred as entity consistency. There are other discourse dependencies that MT fails to capture, such as tense cohesion, ellipsis and coreference. We have left explanations of discourse phenomena to \Cref{subsec:error}.}

% Why Document translation is more than sentence-by-sentence translation?
    % Sentences are parts of texts, and texts have properties beyond those of their individual sentences, including cohesion, coherence and coreference.

% Document-wide properties that are not possible to be captured by sentence-level NMT:
    % document-wide properties, such as style, register, reading level and genre, that are visible in the frequency and distribution of words, word senses, referential forms and syntactic structures;  (purpose/genre/topic, the root of intention structure)
    % patterns of topical or functional sub-structures that mean that frequencies and distributions of words, word senses, referential forms and syntactic structures will vary across a text; (intention)
    % relations between clauses or between referring expressions that can be signaled explicitly or implicitly, that reflect a text's coherence; (attention)
    % frequent appeal to reduced expressions that rely on context to efficiently convey their message. (zero pronouns, pro-drop, attention)

% In the past, we deliberately ignore discourse phenomena in developing MT systems:
    % We still have little idea how to translate into a closely related language like French or German, English sentences containing such words as "he", "she", "it", "not", "and", and "of".  Furthermore, such work as has been done on these problems has been studiously ignored by all those currently involved in developing systems.

Over the past few years, there have been efforts to tackle this problem by building context-aware NMT models~\citep[][\textit{inter alia}]{wang-etal-2017-exploiting, miculicich-2018-hat, maruf-haffari-2018-document, voita-etal-2019-context}. %kuang-etal-2018-modeling, ctx
Although such approaches have achieved some improvements, they nonetheless suffer from a dearth of document level training data. % robustness of those models
Take the WMT news translation task as an example. The document level news commentary corpus~\cite{tiedemann-2012-OPUS} only contains 6.4M tokens while the available sentence-level training data has around 825M tokens.
% Moreover, News articles are normally short and does not contains much discourse phenomena. 
To alleviate this problem, we collect a large document level parallel corpus that consists of 196K paragraphs from Chinese novels translated into English. 
As shown in \Cref{fig:motivation}, it is the largest document-level corpus to the best of our knowledge.
Additionally, an in-depth human analysis shows, it is very challenging for current NMT systems due to its rich discourse phenomena (see \Cref{fig:intro_example}).

To better evaluate context-aware MT models, we further annotate the test set with characteristic discourse-level phenomena, namely ambiguity and ellipsis.
The test set is designed to specifically measure models’ capacity to exploit such long range linguistic context. %for coreference and coherence/cohesion
% parallel documents are too scarce to build robust document-level NMT models. 
% exist three main drawbacks that may restrict development of document-level NMT.
We then conduct systematic evaluations of several baseline models as well as human post-editing performance on the \BWB{} corpus and observe large gaps between NMT models and human performance.
We hope that this corpus will help us understand the deficiencies of existing systems and build better systems for document level machine translation.


% Our contributions are threefold:
% \begin{itemize}
%     \item In order to guide and inspire more work on in the area of document-level MT research, we present the to-date largest parallel corpus. Used for training.
%     \item we present a first evaluation benchmark for document-level MT that large NMT models could be trained on.
%     \item We present a test suite annotated with ambiguity and ellipsis that can be used for evaluation. 
%     \item We conduct systematic evaluations of several baseline models -- both sentence-level and document-level. We also provide human post-editing results as well as human evaluation on this corpus.
% \end{itemize}




==> tabs/datasets.tex <==
\begin{table}[t]
\begin{adjustbox}{width=0.49\textwidth}
{
\centering
\begin{tabular}{l|l|rrr|rrr}
\toprule[2pt]
\multirow{2}{*}{Corpus}  & \multirow{2}{*}{Genre}  & \multicolumn{3}{c|}{Size}                                                                         & \multicolumn{3}{c}{Averaged Length}                    \\
                    &                           & \#word & \#sent & \#doc & \#w/s & \#s/d & \#w/d \\
\midrule[1pt]
	
IWSLT  & TED talk &  4.2M                         & 0.2M                            & 2K                              & 19.5                           & 100                            & 2,100                         \\
NewsCom & news    & 6.4M                         & 0.2M                            & 5K                              & 30.7                           & 40                             & 1,288                         \\
Europarl                & Parliament            & 7.3M                         & 0.2M                            & 15K                             & 35.1                           & 13                             & 485                           \\
LDC                     & News                      &  81.8M                        & 2.8M                            & 61K                             & 23.7                           & 46                             & 1,340                         \\
OpenSub &       Subtitle     &  16.9M                        & 2.2M                            & 3K                              & 5.6                            & 733                            & 5,647                         \\
\midrule[1pt]
\multirow{2}{*}{\BWB}     & novel (chapter)           &  \textbf{460.8M}                       & \textbf{9.6M}                            & \textbf{196K}                            & \textbf{48.1}                          & 49                             & 2,356                         \\
&    novel (book)              &  \textbf{460.8M}                       & \textbf{9.6M}                            & 384                             & \textbf{48.1}                           & \textbf{25.0K}                          & \textbf{1.2M}          \\
\bottomrule[2pt]
\end{tabular}
}
\end{adjustbox}
    \caption{Statistics of various document-level parallel corpora. For corpora that contain multiple language pairs (IWSLT and OpenSub), we report the statistics for ZH-EN. For corpora that do not contain ZH-EN parallel documents (NewsComand and Europarl), we report the statistics of their (largest) available language pairs (DE-EN and ET-EN). \textit{w}, \textit{s} and \textit{d} stand for word, sentence and document, respectively. The full list is in \Cref{tab:datasets_full}.\looseness=-1}
    \label{tab:datasets}
% \vspace{-5pt}
\end{table}

